Joint Deblurring and 3D Reconstruction for Macrophotography

Macro lens has the advantages of high resolution and large magnification, and 3D modeling of small and detailed objects can provide richer information. However, defocus blur in macrophotography is a long-standing problem that heavily hinders the clear imaging of the captured objects and high-quality 3D reconstruction of them. Traditional image deblurring methods require a large number of images and annotations, and there is currently no multi-view 3D reconstruction method for macrophotography. In this work, we propose a joint deblurring and 3D reconstruction method for macrophotography. Starting from multi-view blurry images captured, we jointly optimize the clear 3D model of the object and the defocus blur kernel of each pixel. The entire framework adopts a differentiable rendering method to self-supervise the optimization of the 3D model and the defocus blur kernel. Extensive experiments show that from a small number of multi-view images, our proposed method can not only achieve high-quality image deblurring but also recover high-fidelity 3D appearance.

==> imgs/ablation_visual_comparison.tex <==
%& Ablation Study Visual Comparisons
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \begin{tabular}[b]{cccccccc}
        % \hline
         Novel View & Defocus & w/o depth & w/o mask & w/o stages & w/o BlurNet & Ours & GT\\

        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/marked_grain_gt.png}
            % \caption{Grain}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_grain_defocus.png}
            % \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_grain_no_depth.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_grain_no_mask.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_grain_no_c2f.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_grain_no_blurnet.png}
            % \caption{}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_grain_full.png}
            % \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_grain_gt.png}
            % \caption{}
        \end{subfigure} \\ 

        PSNR/SSIM &  & 33.52/0.926 & 33.43/0.926 & 29.17/0.895 & 34.55/0.939 & \best{34.77}/\best{0.942} & \\

        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/marked_seed_gt.png}
            % \caption{Seed}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_seed_defocus.png}
            % \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_seed_no_depth.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_seed_no_mask.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_seed_no_c2f.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_seed_no_blurnet.png}
            % \caption{}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_seed_full.png}
            % \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_seed_gt.png}
            % \caption{}
        \end{subfigure} \\ 

        PSNR/SSIM &  & 38.87/0.957 & 38.74/0.957 & 29.49/0.884 & 39.82/0.970 & \best{40.26}/\best{0.974} & \\

        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/marked_spider_gt.png}
            % \caption{Grain}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_spider_defocus.png}
            % \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_spider_no_depth.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_spider_no_mask.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_spider_no_c2f.png}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_spider_no_blurnet.png}
            % \caption{}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_spider_full.png}
            % \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.1\linewidth}
            \includegraphics[width=\textwidth]{imgs/ablation_comparison/roi_spider_gt.png}
            % \caption{}
        \end{subfigure} \\ 



        PSNR/SSIM &  & 37.76/0.970 & 37.35/0.965 & \best{38.00}/\best{0.973} & 37.63/0.968 & 37.87/0.972 & \\



        % \hline
    \end{tabular}
    \caption{\textbf{Visual comparisons of ablation studies on synthetic dataset}. Each row shows the results of removing different components from our method: depth input (w/o depth), clarity mask (w/o mask), multi-stage training (w/o stages), and BlurNet architecture (w/o BlurNet). We color code the \best{\textbf{best}} results.}
    \label{fig:ablation_comparison}
    \vspace{-1.5em}
\end{figure*}


==> imgs/rebuttal_qual_comp.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure}[htb!]
% \vspace{-1.5em}
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    % \begin{tabular}[b]{ccccccccc}
    \begin{tabular}[b]{cccccc}
             Test view & Defocus & 3DGS & Restormer & Ours & GT\\

        \begin{subfigure}[b]{0.285\linewidth}
            \includegraphics[width=\textwidth]{imgs/rebuttal_comp/marked_spider_gt.pdf}
            % \caption{mine}
        \end{subfigure} &
        \begin{subfigure}[b]{0.143\linewidth}
            \includegraphics[width=\textwidth]{imgs/rebuttal_comp/defocus_spider.pdf}
            % \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.143\linewidth}
            \includegraphics[width=\textwidth]{imgs/rebuttal_comp/roi_spider_3dgs.pdf}
            % \caption{}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.143\linewidth}
            \includegraphics[width=\textwidth]{imgs/rebuttal_comp/roi_spider_restormer.pdf}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.143\linewidth}
            \includegraphics[width=\textwidth]{imgs/rebuttal_comp/roi_spider_ours.pdf}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.143\linewidth}
            \includegraphics[width=\textwidth]{imgs/rebuttal_comp/roi_spider_gt.pdf}
            % \caption{}
        \end{subfigure} \\ 


        % \hline
    \end{tabular}
    % \vspace{-1.5em}
    \caption{\textbf{Qualitive comparison for objects with complex shape} }
    \label{fig:rebuttal_qual}
    \vspace{-2em}
\end{figure}

% \captionsetup[subfigure]{labelformat=empty}
% \newcommand{\tp}[1]{\colorbox{LimeGreen}{#1}}


==> imgs/sup_visualization.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \begin{tabular}[b]{ccccc}
        % \hline
         Defocus & 3DGS\cite{kerbl20233dgs} & DbGS\cite{lee2024deblurring3dgs} & INIK\cite{quan2023} & Ours \\

        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/syn_comparison/marked_grain_gt.pdf}
            % \caption{Grain}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/syn_comparison/marked_grain_gt.pdf}
            % \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/syn_comparison/marked_grain_gt.pdf}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/syn_comparison/marked_grain_gt.pdf}
            % \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/syn_comparison/marked_grain_gt.pdf}
            % \caption{}
        \end{subfigure}  \\ 
        



        % \hline
    \end{tabular}
    \caption{\textbf{More visual results on our dataset}. The proposed method achieves the best deblur performance on macrophotography datasets. DbGS, Res, and INIK are the shorthands for Deblurring-3DGS, Restormer+3DGS, and INIKNet+3DGS.}
    \label{fig:sup_results}
    \vspace{-1.5em}
\end{figure*}

% \captionsetup[subfigure]{labelformat=empty}
% \newcommand{\tp}[1]{\colorbox{LimeGreen}{#1}}


==> imgs/training_progression_visual.tex <==
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \small
    \begin{tabular}[b]{ccccc}
        
        Iteration 3000 & Iteration 15000 & Iteration 25000 & Iteration 30000 & Ground Truth \\
        
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/ours_03000.png}
            % \caption{3K}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/ours_15000.png}
            % \caption{15K}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/ours_25000.png}
            % \caption{25K}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/ours_30000.png}
            % \caption{30K}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/gt.png}
            % \caption{GT}
        \end{subfigure} \\
        
        \multicolumn{5}{c}{Ours} \\
        
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/3dgs_03000.png}
            % \caption{3K}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/3dgs_15000.png}
            % \caption{15K}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/3dgs_25000.png}
            % \caption{25K}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/3dgs_30000.png}
            % \caption{30K}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{imgs/training_comparison/gt.png}
            % \caption{GT}
        \end{subfigure} \\
        
        \multicolumn{5}{c}{3DGS Baseline} \\
        
    \end{tabular}
    \caption{\textbf{Training progression comparison between our method and 3DGS baseline}. The visualization demonstrates how our method progressively recovers sharp details from blurry inputs across different training iterations, while the 3DGS baseline struggles to achieve clear reconstruction from the same blurry inputs.}
    \label{fig:training_progression}
    \vspace{-1.5em}
\end{figure*}


==> sec/0_abstract.tex <==
\begin{abstract}
Macrophotography for sub-centimeter scale objects offers high resolution, but defocus blur due to shallow depth of field severely hinders clear imaging and high-quality 3D reconstruction. Traditional deblurring methods often require extensive annotations or struggle with multi-view consistency, and current multi-view 3D reconstruction is not tailored for macrophotography's unique blur. This work proposes a novel joint deblurring and 3D reconstruction method specifically for macrophotography. Starting from multi-view blurry images, we jointly optimize a clear 3D model of the object and the per-pixel defocus blur kernels. The framework employs differentiable rendering for self-supervised optimization of both the 3D model and blur kernels. Extensive experiments show that from a small number of multi-view images, our method achieves high-quality image deblurring and recovers high-fidelity 3D appearance, outperforming existing approaches.
\end{abstract}
